Deep Point Cloud Reconstruction

Point cloud obtained from 3D scanning is often sparse, noisy, and irregular. To cope with these issues, recent studies have been separately conducted to densify, denoise, and complete inaccurate point cloud. In this paper, we advocate that jointly solving these tasks leads to significant improvement for point cloud reconstruction. To this end, we propose a deep point cloud reconstruction network consisting of two stages: 1) a 3D sparse stacked-hourglass network as for the initial densification and denoising, 2) a refinement via transformers converting the discrete voxels into 3D points. In particular, we further improve the performance of transformer by a newly proposed module called amplified positional encoding. This module has been designed to differently amplify the magnitude of positional encoding vectors based on the points' distances for adaptive refinements. Extensive experiments demonstrate that our network achieves state-of-the-art performance among the recent studies in the ScanNet, ICL-NUIM, and ShapeNetPart datasets. Moreover, we underline the ability of our network to generalize toward real-world and unmet scenes.

==> sections/7-ethics.tex <==
\section{Ethics Statement}
Point cloud reconstruction aims to increase the quality of 3D point data from scanners. Our research does not involve any soc

==> sections/9-0-common.tex <==
Thank you for the precious comments. Following the reviewer's advice, we revise our initial manuscript as follows:
\begin{itemize}
    \item Elaborate the related works section about a surface reconstruction task.
    \item Clarify the~\Sref{subsec:Point re-localization Network}.
    \item Conduct experiments about possible combinations of three previous papers, which is added in~\Tref{table:metric} of the manuscript and \Tref{table:metric-appendix} in the appendix.
    \item Include description in~\Sref{subsec:Comparison} about the strength of the proposed method, generalization and transferability.
    \item Add more qualitative results in the appendix. 
    \item Describe the precise equations of metrics in the appendix.
    \item \textcolor{blue}{Implementation will be released after the review.}
\end{itemize}
With this revision, the initial manuscript becomes more reasonable, analytic and feasible. We hope that all reviewers are satisfied with the improved quality of the paper.
\textcolor{blue}{For the reviewers' convenience, we include our response letter in the appendix.}





==> sections/9-reviewer1-veKS.tex <==
\question{\textbf{[Writings]}
\quoteReviewer{Q.1-1. The high-level idea makes lots of sense to me. Using voxelization to denoise and complete irregular point cloud is reasonable and smart. Besides, we can sample as many points as we want from a voxel grid to get a dense surface. If possible, the authors could further elaborate on these contributions.}} 

Thank you very much for this positive remark regarding using voxelization for this task. As suggested, we underlined the flexibility offered by our voxel based technique in~\Sref{subsec:Comparison} of the manuscript. This advantage is also highlighted by the quantitative results presented in~\Tref{table:metric} of the manuscript and \Tref{table:metric} of the appendix. These results demonstrate that the number of output points~$\mathcal{P}_\text{out}$ can be adjusted by the hyper-parameters while preserving the overall reconstruction quality.



\question{\textbf{[Baseline]}
\quoteReviewer{Q.1-2. The presented results are great, but the baselines are not very considerate. This paper is arguing that the three tasks should be unified and hence multi-task joint-learning baselines should be considered. The simplest setting is to ensemble all three baselines together in an optimized order. Alternatives contain training each baseline method on all three tasks jointly.}} 

Admittedly, our initial experimental setup was lacking fairness, therefore, we have re-conducted a large set of experiments where all possible combinations between the three baselines have been investigated. The obtained results as visible in~\Tref{table:metric} of the manuscript and \Tref{table:metric-appendix} of the appendix. 
Please take an example with some notations used in the tables in~\Tref{table:metric} of the manuscript. For instance, \textit{PC($r{=}4$)${\rightarrow}$PU($r{=}4$)${\rightarrow}$PD} represents the consecutive operation of point completion, and point upsampling and point denoising under upsampling ratio~$r{=}4$. Note that we also take into account the point completion task since this task also considers point densification on the visible surfaces.

None of the tested configurations is qualitatively nor quantitatively competitive with our point reconstruction technique. It should however be noted that since only $2048$ points have been used as input, the point denoising method~\citep{pcd-score} could not be used before upsampling (because~\citep{pcd-score} requires at least 10,000 points to operate). Thus, we cannot provide results for every single possible combination. Nonetheless, our method still achieves state-of-the-art performance among the possible orders of point denoising/completion/upsample networks.



\question{\textbf{[Multi-task learning]}
\quoteReviewer{Q.1-3. The proposed method should also be evaluated for each single task to demonstrate advantages.}} 

We understand the intention of the reviewer veKS. We guess that the worrying points derive from the reviewer veKS's initial description, \textit{\say{I will use the word **multi-task** to refer to the problem setting in this work, in contrast to the single-task baselines.}} If this paper can be viewed as multi-task learning of three different tasks, it is important to evaluate the results on each single task, such as denoise, densification and completion task.

However, our point reconstruction technique cannot truly be considered as a multi-task learning pipeline. There are two reasons. First, the series of problems (sparsity, noise, and irregularity) are inherently resided in raw point clouds. In real-world point clouds, these problems are completely mixed. Second, we solve the problems in a completely joined manner. As a result, we cannot isolate each individual task since our network does not have dedicated to design task-specific header networks nor task-oriented losses. Moreover, even if we forcefully obtain the results in each single task, it will lack fairness and would not reflect our intention nor the capability of our point reconstruction technique. We hope to have clarified this particular point and that the reviewer will understand the context for which we have designed this point reconstruction strategy combining three tasks at once to resolve the inherent shortcomings of 3D point clouds.



\question{\textbf{[Amplified positional encoding]}
\quoteReviewer{Q.1-4. I am not fully convinced by the story of positional encoding. In the original form, the distance information is already expressed as the frequency of the signal. The magnitude is just redundant information. Why is it important? And what kind of effect it will cause precisely?}} 

We apologize for the confusion. The intuition behind our amplitude positional encoding is the following, \textbf{when to embed high frequency signal?} We are inspired by NeRF~\citep{nerf} where positional encoding results in preserving the high-frequency image signal. In our case, we are facing a different situation. high-frequency signal is not always welcomed. When a voxel needs to move to a distant location, it is better to keep the low frequency signal, which is simply operated by decreasing the amplitude of the positional encoding vector as described in~\Fref{fig:fig_trans} of the manuscript.

Such control is possible since we already know the relative distance between voxels that are estimated from the $1^\text{st}$ stage network. As underlined by the reviewer G4Aq, we believe that our amplified encoding is an important contribution of this work. To better highlight the necessity of this component, we further elaborate the paragraphs about our amplified positional encoding in~\Sref{subsec:Point re-localization Network} of the manuscript.



\question{\textbf{[Generalization]}
\quoteReviewer{Q.1-5. For the tested dataset, especially this synthetic ones (ICL-NUIM), how does the input noise/sparsity/incompleteness are created? ... Also, regular synthetic noise (\eg, Gaussian noise) are much simple than real-world noise. How does the proposed framework deal with real-world noise? ... It is unclear how does this framework work for real-world sparse point clouds (\eg, the remote areas in LiDAR data).}} 

Thank you very much for this remark regarding the transferability of the approach.
As the reviewer veKS mentioned, we train our network only in synthetic/object-scale dataset (ShapeNetPart). Then, without fine-tuning, we utilize the pre-trained weights to measure the quality of reconstruction using unmet point clouds in ScanNet or ICL-NUIM datasets. Despite the domain gap between datasets, we think our network generalizes well toward various real datasets. We conjecture that this transferability can be explained by two dominant reasons.

First, we optimize the nature of the objective function. Indeed improving the proximity-to-surface instead of task-specific losses (such as denoising, densification, and completion) seems to be a more generic and generalizable problem. Regardless of the difference in synthetic and real-world noises, our network is trained to improve the quality of reconstruction. Also, this is clearly different from the point completion task~\citep{pcc-point-completion-net} that concentrates on category-specific datasets for generating points in occluded regions of objects.

Second, we utilize the hash table for sparse convolution layer instead of $k$ Nearest Neighbor. To handle noisy and sparse point cloud, $k$NN is not a proper choice since it is sensitive to the density of point clouds~\citep{interpconv}. Nonetheless, previous studies~\citep{pcu-dispu,pcc-snowflake,pcu-punet} mainly rely on this clustering algorithm. In contrast, sparse convolution layer takes absolute scale of receptive field regardless of the input distribution, which results in better transferability toward unmet and real-world scenes.

Note that we apply random Gaussian noise into ICL-NUIM dataset following~\citep{pcu-dispu}. This synthetic noise is truely much simpler than the real-world noise, as addressed by the reviewer. Since we did not precisely analyze the noise modeling, we have improved the exposition in the paper to clarify the discussion.


\question{\textbf{[Sparse stacked hourglass network]}
\quoteReviewer{Q.1-6. 3D sparse stacked hourglass network is not a super popular network. It is also not implemented in popular sparse conv net framework (\eg, Minkowski engine). Why this network is adopted? Maybe the authors can share some related works to justify the advantage. It is not a common choice.}}

In our understanding, stacked hourglass has unique properties and is widely used for various applications. First of all, we found that the total number of citations of stacked hourglass network is \textbf{3364}~\citep{hourglass} and \textbf{541}~\citep{associative-embedding}. Note that the original stacked hourglass network is proposed in~\citep{hourglass} and the modified version of the network is introduced in~\citep{associative-embedding} by the same first author. 

Moreover, the variants of stacked hourglass network largely used in various tasks. For instance in stereo matching network, PSMNet (cite:~\textbf{706})~\citep{psmnet}, GANet (cite:~\textbf{246})~\citep{ganet-stereo}, AANet (cite:~\textbf{76})~\citep{aanet-stereo}, utilizes a volumetric version of hourglass network using 3D CNNs. This paper clearly mentions their stacked hourglass network in their abstract, \textit{"The 3D CNN learns to regularize cost volume using stacked multiple hourglass networks in conjunction with intermediate supervision."} In another example, multi-view stereo task, DPSNet (cite:~\textbf{98})~\citep{dpsnet}  also adopts 3D stacked hourglass network to aggregate cost volumes. Different from deep and wide U-shape network, such as Minkowski-UNet~\citep{minkowski}, using multiple light encoder-decoder networks (\ie, stacked hourglass network) aims to sequentially refine feature vectors by intermediate losses.

In summary, our $1^\text{st}$ stage network aims to sequentially refine the given point cloud through the proposed sparse stacked hourglass network. Similar to the idea of voxel carving, hourglass networks re-shape the sparse points in a coarse-to-fine manner. We hope that the reviewer veKS is satisfied with our understanding of stacked hourglass network~\citep{hourglass}. Also, we expect the future studies about point cloud reconstruction will widely use this sparse version of stacked hourglass network as stereo matching methods~\citep{psmnet,aanet-stereo,ganet-stereo} and multi-view stereo~\citep{dpsnet,volumefusion} studies do.



\question{\textbf{[Missing details]}
\quoteReviewer{Q.1-7. How many voxels are processed in the transformer on average?}} 

We apologize for the missing details. We set $k=8$ as an input of our transformer. This information is included in~\Sref{subsec:Point re-localization Network} of the manuscript and \Tref{table:metric-appendix} of the appendix.



\question{\textbf{[Missing details]}
\quoteReviewer{Q.1-8. How is the dimension of $\mathcal{P}_\text{out}$ decided?}} 

Since our $1^\text{st}$ stage network adaptively generates and prunes voxels, we cannot precisely decide for the dimension of $\mathcal{P}_\text{out} {\in} \mathbb{R}^{N'{\times}3}$ where $N'$ is determined after the inference. Thus, we report the average cardinality of the generated point clouds in~\Tref{table:metric} of the manuscript.



\question{\textbf{[Related works]}
\quoteReviewer{Q.1-9. The difference between point upsampling and point completion is not very clear. The very specific definition should be made in the very early stage of the writing so that there is no ambiguity between the challenges that these two problems pose.
}} 
% Besides, the experimental results should clearly demonstrate how does the proposed framework address each sub-problem (above two+denoising) individually. Unfortunately, these results are either missing or not very clear right now.

The difference between the different tasks has been described in the "related works" section. The goal of point upsampling is to densify sparse but homogeneously distributed input points. On the other hand, the point completion task, as described in the pioneering paper~\citep{pcc-point-completion-net}, aims at extrapolating entire parts of the objects resulting from occlusions or the limited sensor resolution. Regarding the experiments validating each task, we invite the reviewer to refer to our response entitled ``Multi-task learning" in this rebuttal.



\question{\textbf{[Title]}
\quoteReviewer{Q.1-10. If find it misleading to their this task \emph{point cloud reconstruction}. A maybe improper analogy is that we do not call joint image denoising and super-resolution and image generation. If the authors really want to use the term reconstruction, maybe call it \emph{conditioned point cloud reconstruction}? Or something else that is more accurate like \emph{point cloud refinement}?}}

We are pleased for the reviewer's recommendation. We also think of this naming issue before the submission. Our conclusion is that we put more weights on the quality of 3D reconstruction using 3D points, so called point cloud reconstruction. As addressed by the reviewer~\textbf{dx4y}, this task can be similar to surface reconstruction task because of the common goals, high-quality 3D description. However, without point triangulation or mesh formulation, this task truely focuses on the point itself to describe 3D environments. We hope that the reviewer is satisfied with our opinion.



\question{\textbf{[Missing details]}
\quoteReviewer{Q.1-11. Where are the cluster information used in the later framework? If I understand correctly, this used because the voxel-to-point step only operates on center voxels and hence we want a locally augmented feature representation?}} 

To be more informative, we revise the paragraphs in~\Sref{subsec:Point re-localization Network}. 

Let us describe the detailed process in the point re-localization network, which is illustrated in~\Fref{fig:fig_trans}. Given output voxels~$\mathcal{V}_\text{out}$, we collect the $K({=}8)$ closest voxels to each voxel~$\mathbf{v}_i{\in}\mathbb{R}^{1{\times}3}$ using the hash table that we used in the $1^\text{st}$ stage network. Then, we obtain a voxel set~$\mathcal{V}_i{=}\{\mathbf{v}_k\}_{k{=}1}^{K}$ that is referenced to the query voxel~$\mathbf{v}_i$. Similarly, we cluster a set of voxel features~$\mathcal{F}_i{=}\{\mathbf{f}_k\}_{k{=}1}^{K}$ that correspond to~$\mathcal{P}_i$. As in~\Fref{fig:fig_trans}, the $2^\text{nd}$ stage network regresses the location of a query point~$\mathbf{p}_i$ (red voxel) using the geometric relation between the query voxel~$\mathbf{v}_i$ and its neighbor~$\mathcal{V}_i$ (white voxels) through self/cross attention layers.

While this formulation is close to PointTransformer~\citep{point-transformer}, our point re-localization network has three distinctive differences. First, PointTransformer utilizes $k$-Nearest Neighbors to group 3D points, we re-use the voxel hashing that is computed in the previous stage. Second, our network consists of both self-attention and cross-attention. In our analysis, it is better to use two different attention layers than to solely adopt self-attention. 




\question{\textbf{[Figure]}
\quoteReviewer{Q.1-12. Fig2 input figure is barely visible.}}

We are sincerely thankful regarding this comment on the editorial quality of the paper.  In~\Fref{fig:fig_arch} of the manuscript, to faithfully highlight the ability of our network, we intentionally set the same point's size for the visualization of the input and output point clouds. This clearly emphasizes how precisely and densely our network reconstructs the given sparse points. To clarify this point, we include more details about visualization in~\Fref{fig:fig_arch} of the manuscript.



\question{\textbf{[highlight]}
\quoteReviewer{Q.1-13. In Tab.1, maybe the light color can be used to highlight the 2nd best among the baseline method. Highlighting the 2nd best among all including **ours** cannot fully demonstrate the advantages.}}

Following the request by the reviewer, we remove the $2^\text{nd}$ best highlight in~\Tref{table:metric} of the manuscript.



==> sections/9-reviewer2-1Mes.tex <==
\question{\textbf{[More qualitative results]}
\quoteReviewer{Q2-1. Qualitative examples are good and would like to see more of them in the supplemental material.}} 

We newly include qualitative results in the appendix. Also, we update the results from sequential uses of three baselines in~\Fref{fig:fig_qual} of the manuscript.



\question{\textbf{[Amplified positional encoding]}
\quoteReviewer{Q2-2. The initial section of the paper until sec.$3.1$ is clear and well explained, while section 3.2 needs a better explanation. I still do not understand the exact intuition behind the amplitude-based positional embedding.}} 

We newly revise section~$3.2$ of the manuscript following the reviewer's comment. The intuition behind our amplitude positional encoding is clear, \textbf{when to embed high frequency signal?} We are inspired by NeRF~\citep{nerf} where positional encoding results in preserving the high-frequency image signal. In our case, we are in a different situation. high-frequency signal is not always welcomed. When a voxel needs to move to a distant location, it is better to keep the low frequency signal, which is simply conducted by decreasing the amplitude of the positional encoding vector as in~\Fref{fig:fig_trans} of the manuscript.

Such control is possible since we already know the relative distance between voxels that are estimated from the $1^\text{st}$ stage network. As underlined by the reviewer G4Aq, we believe that our amplified encoding is an important contribution of this work. To better highlight the necessity of this component, we further elaborate the paragraphs about our amplified positional encoding in~\Sref{subsec:Point re-localization Network} of the manuscript.




\question{\textbf{[Writing]}
\quoteReviewer{Q2-3. The baselines are not explained well, the exact characteristics of the Snowflake-PC $\rightarrow$ Score-PD are not explained, likewise for Dis-PU. These sections need rewriting.}}

As requested by the reviewer, we revised~\Sref{subsec:Baseline Approaches} and \Sref{sec:Related Works} of the manuscript. Also, we included additional experiments about ensembles of three related papers in~\Tref{table:metric} of the manuscript and~\Tref{table:metric-appendix} in the appendix. Let us present the revised paragraphs in~\Sref{subsec:Baseline Approaches} below.

In particular, we analyze the efficacy of ours compared to the combination of the existing studies. For instance in~\Tref{table:metric}, \textit{PC($r{=}4$)${\rightarrow}$PU($r{=}4$)${\rightarrow}$PD} represents consecutive operation of point completion, and point upsampling and point denoising under upsampling ratio~$r{=}4$. Note that we also take into account the point completion task since this task also considers point densification on visible surface.



\question{\textbf{[Details]}
\quoteReviewer{Q2-4. There is no evaluation independently for Stage-1 all evaluations. ... I understand that maybe doing the full evaluation on Stage-1 is not possible.}}

The evaluation for our $1^\text{st}$ network is already included in~\Tref{table:ablation-arch}-(\textcolor{blue}{b}) of the manuscript. For clarity, we denote the name as $1^\text{st}$ stage.  



\question{\textbf{[Details]}
\quoteReviewer{Q2-5. The paper claims like past work when they upsample they do not have this scaling-up factor of $r$ but I think in this case, $r$ just manifests as the voxel density in stage 1.}}

It is true that the \emph{generative sparse transposed convolution layer} densifies voxels in a fixed ratio~$r$. Following the reviewer's comment, we revise the sentences in~\Sref{subsec:Voxel Generation Network} of the manuscript. 



\question{\textbf{[Future direction]}
\quoteReviewer{Q2-6. I am also not clear what happens when multiple voxel centers move to the same location in 3D points.}}

We are pleased to answer this very well spotted observation. This is, indeed, a limitation of our architectural design. Specifically, when multiple points are closer than the voxel size, they are merged into a single voxel during the voxelization process. Although this was not clearly visible in our experiments, we agree that the raised concerns can harm the results. In the future, we think of a new network design that utilizes both voxel and point-level understanding to overcome such limitations.


==> sections/9-reviewer3-G4Aq.tex <==
\question{\textbf{[Generalization]}
\quoteReviewer{Q3-1. It would be better if the paper could explain why the proposed new method can achieve such strong generalization ability, and why the generalization ability of the existing methods is poor.}} 

It is our pleasure for the reviewer to recognize the strength of our method, generalization.
We conjecture that this transferability can be explained by two dominant reasons.

First, we optimize the nature of the objective function. Indeed improving the proximity-to-surface instead of task-specific losses (such as denoising, densification, and completion) seems to be a more generic and generalizable problem.
Regardless of the difference in synthetic and real-world noises, our network is trained to improve the quality of reconstruction. Also, this is clearly different from the point completion task~\citep{pcc-point-completion-net} that concentrates on category-specific datasets for generating points in occluded regions of objects.

Second, we utilize the hash table for sparse convolution layer instead of $k$ Nearest Neighbor. To handle noisy and sparse point cloud, $k$NN is not a proper choice since it is sensitive to the density of point clouds~\citep{interpconv}. Nonetheless, previous studies~\citep{pcu-dispu,pcc-snowflake,pcu-punet} mainly rely on this clustering algorithm. In contrast, sparse convolution layer takes absolute scale of receptive field regardless of the input distribution, which results in better transferability toward unmet and real-world scenes.

These are our analyses of our strength in better generalization and transferability. With our sparse stacked hourglass network, we can achieve well-generalized reconstruction performance. These voxelized results are further refined by the $2^\text{nd}$ stage network that converts discrete voxels into 3D points.

Finally, we revised \Sref{subsec:Comparison} of the manuscript to clarify the discussion about generalization and transferability of our deep point cloud reconstruction network.

==> sections/9-reviewer4-dx4y.tex <==
\question{\textbf{[Point cloud reconstruction]}
\quoteReviewer{Q4-1. Since many scans are combined into a single scan, there is another challenge that is entirely overlooked, misalignment. If the idea is to combine all challenges into one, this should another challenge to address.}} 

Point cloud registration is another topic that is widely addressed in previous studies~\citep{deep-global-registration,deep-icp,gojcic2020learning}. However, in our opinion, point cloud registration (misalignment) is not an inherent problem of point clouds. Misalignment usually derives from the extrinsic parameters between multiple 3D scans. In our point of view, this problem happens when we fuse multiple 3D scans that are taken in different views or time stamps. We think that it will be a wonderful future direction that extends the applicability of point cloud reconstruction toward multiple 3D scans.



\question{\textbf{[Related works]}
\quoteReviewer{Q4-2. Missing related work. There is a very large body of recent works on neural shape implicit representation which focus on the surface reconstruction task.  ..., one could simply sample points on the zero level set and achieve point cloud reconstruction.}} 

We apologize for the missing references about surface reconstruction. Following the reviewer's advice, we included a paragraph in~\Sref{sec:Related Works}. However, we claim that the point cloud reconstruction task is clearly different from surface reconstruction. Let us briefly describe their difference.

First, mesh triangulation is not related to the inherent shortcomings of point cloud. According to the recent papers, PointTriNet~\citep{point-tri-net} and \citep{learning-delaunay}, conventional studies about point triangulation often require dense and uniform 3D points. It implies that the surface reconstruction task puts more weight on mesh generation from given 3D points.


Second, according to the DeepSDF~\citep{deepsdf}, this paper also utilizes ShapeNet dataset~\citep{shapenet}, but relies on a large number of points for training, which is described as \textit{\say{To prepare data, we start by normalizing each mesh to a unit sphere and sampling \textbf{500,000} spatial points x’s: we sample more aggressively near the surface of the object as we want to capture a more detailed SDF near the surface}}. Therefore, while being different, we believe that our research can be very complementary with such type of work. For instance, point cloud reconstruction can be applied as a pre-processing to provide a dense and well distributed point cloud to train DeepSDF.

Third, point sampling from mesh cannot be ahead of point cloud reconstruction task. In our case, we utilize Poisson Disk Sampling~\citep{poisson-disk-sampling,open3d} to obtain ground truth point cloud from ground truth mesh provided in the ShapeNet dataset~\citep{shapenet,shapenet-part}.

Based on these three reasons, we claim that point cloud reconstruction has clear characteristics compared to the surface reconstruction task. Moreover, to obtain such a large amount of points to train recent implicit methods~\citep{deepsdf}, point cloud reconstruction should be taken as a pre-processing stage, ahead of surface reconstruction. We hope the reviewer is satisfied with the necessity of point cloud reconstruction task.




\question{\textbf{[Details]}
\quoteReviewer{Q4-3. It was not clear to me how the final number of points is specified. Also, not clear how color information is determined for the newly generated points.}} 

As we described in~\Sref{subsec:Voxel Generation Network}, our network jointly generates and prunes voxels in an adaptive manner. Even though transposed generative convolution layer upsamples voxels in a fixed ratio of $r$, voxel pruning layer removes outliers based on their signals. Thus, we cannot strictly say the number of outputs and report the average of $\mathcal{P}_\text{out}$ in~\Tref{table:metric}.



\question{\textbf{[Evaluation]}
\quoteReviewer{Q4-4. I find the choices of the baseline questionable. First, there was no unified approach used (denoising + completion + sampling). Second, It would make more sense to me compare the proposed method on the other's task since it is expected that a denoising method will not do well for upsampling. Third, in the combined baselines (Snowflake-PC $\rightarrow$ Score-PD and Dis-PU $\rightarrow$ score-PD), it is not clear the order of application (it makes sense to first denoise and upsample/complete but the text suggest the opposite which should be reported). Finally, as mentioned in the related work, the paper lacks comparison to implicit representations surface reconstruction.}} 

Following the request of the reviewers, we conduct additional experiments about the combination of the three models, denoising, completion and upsampling. It turns out that the different orders of three models do not improve the quality of point reconstruction compared to the results in~\Tref{table:metric} of the manuscript. We claim that these results consistently support the necessity of a joint solution for point cloud reconstruction.

We think that our point reconstruction technique cannot truly be considered as a multi-task learning pipeline since it solves the problems in a completely joined manner. As a result, we cannot isolate each individual task since our network does not have dedicated to design task-specific header networks nor task-oriented losses. Instead, we assume that these problems are inherent to point cloud obtained by scanning devices and should be resolved together. Moreover, even if we forcefully obtain the results in each single task, it will lack fairness and would not reflect our intention nor the capability of our point reconstruction technique. We hope to have clarified this particular point and that the reviewer will understand the context for which we have designed this point reconstruction strategy combining three tasks at once to resolve the inherent shortcomings of 3D point clouds.



% \question{\textbf{[Dataset]}
% \quoteReviewer{Q4-05. The chosen datasets are commonly used and an understandable choice for this task. However, they are strongly biased towards planar geometries. I expect to see results on the surface reconstruction benchmark which is small but has a mix of complex geometries.}}
% \JS{@TBU}



\question{\textbf{[Novelty]}
\quoteReviewer{Q4-5. This paper is missing an important subsection that provides some insight into what the different modules have learned and what is that beneficial to the task. This raises some questions about novelty - how is this approach better than the sum of its technical parts?}}

\input{table/metrics/table-metric-for-appendix}

As noted by three reviewers (veKS, 1Mes, and G4Aq), our contributions derive from a two-stage pipeline that aims to handle raw point clouds via voxelization. This module is very simple and straightforward, but as we describe in~\Sref{subsec:Voxel Generation Network}, each layer are deeply related to the point cloud reconstruction task. This architectural design leads to better generalization and transferability toward unmet and real-world 3D scans as in~\Tref{table:metric-for-appendix}. Let us briefly explain the reasons behind our strength of generalization and transferability. Throughout this paper, we conjecture that this transferability can be explained by two dominant reasons.

First, we optimize the nature of the objective function. Indeed improving the proximity-to-surface instead of task-specific losses (such as denoising, densification, and completion) seems to be a more generic and generalizable problem. Regardless of the difference in synthetic and real-world noises, our network is trained to improve the quality of reconstruction. Also, this is clearly different from the point completion task~\citep{pcc-point-completion-net} that concentrates on category-specific datasets for generating points in occluded regions of objects.

Second, we utilize the hash table for sparse convolution layer instead of $k$ Nearest Neighbor. To handle noisy and sparse point cloud, $k$NN is not a proper choice since it is sensitive to the density of point clouds~\citep{interpconv}. Nonetheless, previous studies~\citep{pcu-dispu,pcc-snowflake,pcu-punet} mainly rely on this clustering algorithm. In contrast, sparse convolution layer takes absolute scale of receptive field regardless of the input distribution, which results in better transferability toward unmet and real-world scenes.

Nonetheless, we find that we need to further provide a reasonable analysis of our strength in generalization ability and transferability. Following the advice from the reviewer dx4y, we elaborate the strength of our method in~\Sref{subsec:Comparison} of the manuscript. 




\question{\textbf{[Writing]}
\quoteReviewer{Q4-6. In its current form, the paper is not self-contained and the method is not reproducible due to a lack of technical details}}

Following the request from the reviewer, we newly update \Fref{fig:fig_hourglass} and \Fref{fig:fig_trans}. Every detail of channel dimensions and connectivity between layers is precisely described. Moreover, we are planning to release the code after the review. Since this is a pioneering paper that opens a new task, as a researcher, we think it is our responsibility to clearly open everything for the community.



\question{\textbf{[Minor-Writing]}
\quoteReviewer{Q4-7. There is an issue with the term "continuous 3D points" which repeats itself in the paper. Point clouds are not continuous, they are sampled on a continuous surface.}}

We apologize for the confusing terminology. We revise all these words in the manuscript.




\question{\textbf{[Minor-Metrics]}
\quoteReviewer{Q4-8. The evaluation metrics were not properly specified. When performing standardized experiments it may be sometimes acceptable to commit this, however, in these cases, the paper proposes a new task, therefore the evaluation metrics should be specified.}}

Following the request by the reviewer, we describe the precise equations of all metrics that we used in the appendix. 

\question{\textbf{[Minor-Metrics]}
\quoteReviewer{Q4-9. $\mathcal{V}_\text{mid}$ is missing.}}

We apologize for the missing details. Following the reviewer's request, we newly update the~\Fref{fig:fig_hourglass} of the manuscript. Note that $\mathcal{V}_\text{mid}$ is the intermediate results from each hourglass network in the $1^\text{st}$ stage network.






==> sections/notation.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}


==> table/metrics/repository/init-submission/table_icl-nuim.tex <==

\resizebox{1.00\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}

\Xhline{2\arrayrulewidth}

\multicolumn{15}{c}{ICL-NUIM dataset} \\ 

\Xhline{2\arrayrulewidth}

\multirow{2}{*}{Methods} 
& \multirow{2}{*}{$\mathcal{P}_\text{in}$}
& \multirow{2}{*}{$\mathcal{P}_\text{out}$}
& & \multicolumn{3}{c}{$k$ Nearest Chamf.~($\downarrow$)} 
& & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<0.5$)} 
& & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<1.0$)} 
% & & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<2l_\text{vox}$)} 

\\ \cline{5-7} \cline{9-11} \cline{13-15} % \cline{19-21} 

& 
& 
& & $k$=1 & $k$=2 & $k$=4 
& & Acc. & Comp. & \textit{f}-score 
& & Acc. & Comp. & \textit{f}-score 
% & & Acc. & Comp. & \textit{f}-score 
\\ 
 
\Xhline{2\arrayrulewidth}


\textcolor{teal}{PC} ($r\text{=}8$)
& 4098 
& 32768
& & 3.32 & 3.59 & 3.97
& & 21.61 & 12.28 & 13.87
& & 44.32 & 50.18 & 45.98
% & & 73.77 & 90.47 & 81.10
\\ 
\textcolor{teal}{PC} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD} 
& 4098 
& 32768
& & 3.21 & 3.40 & 3.69
& & 28.84 & 15.54 & 18.89
& & 56.27 & 48.97 & 51.88
% & & 83.44 & 80.94 & 82.10
\\ 
\textcolor{cyan}{PU} ($r\text{=}8$) 
& 4096 
& 32768
& & {3.25} & {3.49} & {3.86}
& & {21.00} & 13.05 & {14.16}
& & {43.31} & 42.44 & {41.46}
% & & {71.73} & {77.04} & {73.96}
\\
\textcolor{cyan}{PU} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD} 
& 4098 
& 32768
& & 2.85 & 3.09 & 3.45
& & 32.34 & 20.03 & 22.75
& & 61.38 & 51.12& 54.96
% & & 88.94 & 78.86 & 83.38
\\ 
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0100$) 
& 4096
& 21395
&  & \first{1.50} & \first{1.61} & \first{1.79}
&  & \first{75.81} & \first{48.13} & \first{58.44}
&  & \first{92.99} & \first{74.57} & \first{82.40}
% &  & \first{98.83} & \first{87.58} & \first{92.71}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0085$)
& 4096
& 30986
&  & \second{1.70} & \second{1.81} & \second{2.00}
&  & \second{71.65} & \second{46.43} & \second{55.74}
&  & \second{91.01} & \second{72.36} & \second{80.12}
% &  & \second{98.31} & \second{85.31} & \second{91.13}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\




\hline




\textcolor{brown}{PC} ($r\text{=}16$)
& 4098 
& 65536
& & 3.41 & 3.63 & 3.95
& & 18.69 & 17.53 & 16.65
& & 38.26 & 63.02 & 47.20
% & & 65.95 & 93.28 & 77.09
\\ 
\textcolor{brown}{PC} ($r\text{=}16$) ${\rightarrow}$ \textcolor{purple}{PD} 
& 4098 
& 65536
& & 3.18 & 3.34 & 3.59
& & 24.46 & 20.88 & 21.53
& & 50.98 & 57.43 & 53.84
% & & 81.21 & 83.62 & 82.30
\\ 
\textcolor{blue}{PU} ($r\text{=}16$) 
& 4096 
& 65536
& & 3.83 & 4.03 & 4.33 
& & 17.78 & {18.19} & 16.83 
& & 35.45 & {49.93} & 41.03
% & & 59.20 & {82.30} & 68.49 
\\
\textcolor{blue}{PU} ($r\text{=}16$) ${\rightarrow}$ \textcolor{purple}{PD} 
& 4098 
& 65536
& & 2.80 & 3.00 & 3.29
& & 27.46 & 27.11 & 26.18
& & 53.15 & 60.50 & 56.26
% & & 80.82 & 84.31 & 82.35
\\
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0075$) 
& 4096
& 41322
&  & \first{1.87} & \first{1.99} & \first{2.18}
&  & \first{67.78} & \first{44.97} & \first{53.36} 
&  & \first{89.09} & \first{70.52} & \first{78.141}
% &  & \first{97.76} & \first{83.47} & \first{89.78} 
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0065$) 
& 4096
& 56902
&  & \second{2.14} & \second{2.26} & \second{2.45}
&  & \second{63.40} & \second{42.85} & \second{80.26}
&  & \second{86.84} & \second{67.78} & \second{75.41}
% &  & \second{96.08} & \second{80.72} & \second{87.79}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0050$)
& 4096 
& 99321
& & {2.78} & {2.92} & {3.10}
& & {54.11} & {38.09} & {43.55} 
& & {81.76} & {61.88} & {69.45}
% & & {95.68} & {74.77} & {83.38} 
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\

\Xhline{4\arrayrulewidth}

\end{tabular}
}



==> table/metrics/repository/init-submission/table_scannet.tex <==

\resizebox{1.00\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}

\Xhline{2\arrayrulewidth}

\multicolumn{15}{c}{ScanNet dataset} \\ 

\Xhline{2\arrayrulewidth}

\multirow{2}{*}{Methods} 
& \multirow{2}{*}{$\mathcal{P}_\text{in}$}
& \multirow{2}{*}{$\mathcal{P}_\text{out}$}
& & \multicolumn{3}{c}{$k$ Nearest Chamf.~($\downarrow$)} 
& & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<0.5$)} 
& & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<1.0$)} 
% & & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<2l_\text{vox}$)} 

\\ \cline{5-7} \cline{9-11} \cline{13-15} % \cline{19-21} 

& 
& 
& & $k$=1 & $k$=2 & $k$=4 
& & Acc. & Comp. & \textit{f}-score 
& & Acc. & Comp. & \textit{f}-score 
% & & Acc. & Comp. & \textit{f}-score 
\\ 
 
\Xhline{2\arrayrulewidth}

\textcolor{teal}{PC} ($r\text{=}8$)
& 4098 
& 32768
& & {3.64} & {3.98} & {4.43}
& & 19.50 & 8.06 & 10.53
& & 45.32 & {40.23} & 41.19
% & & 74.91 & {86.60} & {80.29}
\\ 
\textcolor{teal}{PC} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD}
& 4098 
& 32768
& & 3.61 & 3.84 & 4.19
& & {24.58} & {10.33} & {13.82}
& & {55.21} & 38.18 & {44.47}
% & & {83.83} & {73.48} & 78.18
\\ 
\textcolor{cyan}{PU} ($r\text{=}8$) 
& 4096
& 32768
& & {3.20} & {3.49} & {3.92}
& & {21.52} & 9.323 & 11.94 
& & {48.30} & 36.10 & {39.72}
% & & {77.34} & 73.12 & {74.70}
\\ 
\textcolor{cyan}{PU} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD}
& 4098 
& 32768
& & 3.01 & 3.29 & 3.71
& & 30.24 & 14.07 & 18.04
& & 63.36 & 42.15 & 49.68
% & & 91.02 & 72.86 & 80.65
\\ 
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0100$)
& 4096
& 27740
&  & \first{1.51} & \first{1.64} & \first{1.87}
&  & \first{70.49} & \first{40.59} & \first{51.29}
&  & \first{93.63} & \first{73.24} & \first{82.02}
% &  & \first{99.23} & \first{88.64} & \first{93.56}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23 
\\ 
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0085$)
& 4096
& 41022
&  & \second{1.73} & \second{1.86} & \second{2.05}
&  & \second{63.67} & \second{38.55} & \second{47.77}
&  & \second{91.03} & \second{70.67} & \second{79.36}
% &  & \second{98.99} & \second{86.43} & \second{92.17}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\





\hline







\textcolor{brown}{PC} ($r\text{=}16$)
& 4098 
& 65536
& & {3.79} & {4.08} & {4.48}
& & 16.91 & 11.96 & 13.12
& & 40.45 & {53.70} & 45.45
% & & 69.45 & {91.12} & {78.69}
\\ 
\textcolor{brown}{PC} ($r\text{=}16$) ${\rightarrow}$ \textcolor{purple}{PD}
& 4098 
& 65536
& & 3.71 & 3.93 & 4.23
& & {21.93} & {15.05} & {17.33}
& & {51.57} & 47.38 & {49.12}
% & & {82.02} & 77.64 & 79.66
\\ 
\textcolor{blue}{PU} ($r\text{=}16$) 
& 4096 
& 65536
& & 3.68 & 3.94 & 4.32 
& & 16.81 & {13.48} & 13.90 
& & 37.89 & {44.60} & 40.04
% & & 63.42 & {80.97} & 70.76 
\\
\textcolor{blue}{PU} ($r\text{=}16$) ${\rightarrow}$ \textcolor{purple}{PD}
& 4098 
& 65536
& & 2.86 & 3.10 & 3.44
& & 26.06 & 21.04 & 22.36
& & 55.73 & 53.56 & 54.04
% & & 83.92 & 80.72 & 82.06
\\ 
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0075$)
& 4096
& 55188
&  & \first{1.91}  & \first{2.04}  & \first{2.24}
&  & \first{57.88} & \first{36.83} & \first{44.72}
&  & \first{88.06} & \first{68.34} & \first{76.72}
% &  & \first{98.46} & \first{84.39} & \first{90.74}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23 
\\
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0065$)
& 4096
& 76182
&  & \second{2.17}  & \second{2.32}  & \second{2.32}
&  & \second{51.55} & \second{34.78} & \second{41.16}
&  & \second{84.47} & \second{65.28} & \second{73.37}
% &  & \second{97.87} & \second{81.53} & \second{88.78}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23 
\\
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0050$)
& 4096
& 116266
& & {2.86}  & {3.02}  & {3.26}
& & {40.42} & {30.24} & {34.08}
& & {76.37} & {58.12} & {65.61}
% & & {96.04} & {74.57} & {83.67}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23 
\\

\Xhline{4\arrayrulewidth}

\end{tabular}
}


==> table/metrics/repository/init-submission/table_shapenet.tex <==
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}

\Xhline{4\arrayrulewidth}
\multicolumn{15}{c}{ShapeNet-Part dataset} \\ 
\Xhline{2\arrayrulewidth}

\multirow{2}{*}{Methods} 
& \multirow{2}{*}{$\mathcal{P}_\text{in}$}
& \multirow{2}{*}{$\mathcal{P}_\text{out}$}
& & \multicolumn{3}{c}{$k$ Nearest Chamf.~($\downarrow$)} 
& & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<0.5$)} 
& & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<1.0$)} 
% & & \multicolumn{3}{c}{Percentage~($\uparrow$) ($<2l_\text{vox}$)} 

\\ \cline{5-7} \cline{9-11} \cline{13-15} % \cline{19-21} 

&  
&  
& & $k$=1 & $k$=2 & $k$=4 
& & Acc. & Comp. & \textit{f}-score 
& & Acc. & Comp. & \textit{f}-score 
% & & Acc. & Comp. & \textit{f}-score 
\\ 
 
\Xhline{2\arrayrulewidth}
PC ($r\text{=}4$)
& 2048 
& 8192
& & \first{1.14} & \first{1.29} & \first{1.51}
& & \second{72.28} & \first{42.71} & \second{51.51}
& & \second{92.41} & \first{88.48} & \first{90.16}
% & & \second{99.14} & \first{98.43} & \first{98.77}
\\ 
PU ($r\text{=}4$) 
& 2048
& 8192
& & 1.56 & 1.69 & 1.90 
& & 60.71 & 26.91 & 36.04  
& & 86.67 & 68.19 & 75.60 
% & & 96.32 & 94.19 & 95.11 
\\ 
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0200$)
& 2048
& 8732
& & \second{1.19} & \second{1.33} & \second{1.52}
& & \first{81.02} & \second{40.41} & \first{53.48} 
& & \first{96.95} & \second{81.23} & \second{88.08} 
% & & \second{99.46} & \first{93.90} & \second{96.49} 
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23 
\\ 







\hline










\textcolor{teal}{PC} ($r\text{=}8$)
& 2048 
& 16384
& & \second{1.01} & \second{1.13} & \second{1.31}
& & 70.89 & \second{60.66} & \second{64.17}
& & {92.16} & \second{93.56} & \second{92.76}
% & & 99.46 & \first{99.41} & \first{99.42}
\\ 
\textcolor{teal}{PC} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD}
& 2048 
& 16384
& & 1.25 & 1.34 & 1.49
& & 61.11 & 42.98 & 49.74
& & 91.73 & 81.01 & 85.83
% & & \first{99.66} & 97.45 & 98.52
\\ 
% \textcolor{teal}{PC} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD}
% &  
% & 
% & & & & 
% & & & & 
% & & & & 
% % & & \first{99.66} & 97.45 & 98.52
% \\ 
\textcolor{cyan}{PU} ($r\text{=}8$) 
& 2048
& 16384
& & {1.02} & {1.14} & {1.32}
& & \second{80.84} & {50.36} & {60.74}
& & \second{95.69} & {82.21} & 88.05
% & & \second{99.57} & {96.69} & {98.07}
% 211017__up_ratio_8__network_DisPU__run_postech2_23
\\
\textcolor{cyan}{PU} ($r\text{=}8$) ${\rightarrow}$ \textcolor{purple}{PD} 
& 2048 
& 16384
& & 1.29 & 1.39 & 1.56
& & 71.79 & 43.88 & 53.57
& & 94.68 & 75.41 & 83.55
% & & 99.65 & 92.70 & 95.95
\\ 
\textcolor{red}{Ours} ($l_\text{vox}\text{=}0.0150$)
& 2048
& 15863
& & \first{0.90}  & \first{0.94}  & \first{1.12}
& & \first{85.77} & \first{69.01} & \first{78.14}
& & \first{97.11} & \first{94.98} & \first{96.16}
% & & \second{99.59} & \second{99.14} & \first{99.42}
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23 
\\
\Xhline{4\arrayrulewidth}

\end{tabular}
}


==> table/metrics/repository/old/ablation-ape.tex <==
\begin{table}[!t]
% \centering
\begin{tabular}{lccccccccc}

\Xhline{2\arrayrulewidth}

\multirow{2}{*}{Method} &  &\multicolumn{3}{c}{Type of positional encoding} & & \multicolumn{4}{c}{Performance} \\ \cline{3-5} \cline{7-10} 
 & & \ \ PE* \ \ &  \ \ PE** \ \ & \ AmpPE (ours) \ & & Chamf. & Acc. & Comp. & \textit{f}-score \\ 
 
\Xhline{2\arrayrulewidth}

Graph-PD &  &  &  &  &  &  & & &  \\
Dis-PU &  &  &  &  &  &  &  & & \\ 
Ours &  &  &  &  &  &  &  & & \\ 

\Xhline{2\arrayrulewidth}

\end{tabular}
\vspace{-2mm}
\caption{\textbf{Ablation study of our amplified positional encoding (AmPE).} Note that PE* represents positional encoding from the original transformer~\cite{point-transformer}, PE** indicates positional encoding from NeRF~\cite{nerf} and AmpPE is the amplified positional encoding.}
\end{table}

==> table/metrics/repository/old/ablation-arch.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{cccccccccc}

\Xhline{2\arrayrulewidth}

\multirow{2}{*}{Method} & & \multicolumn{3}{c}{preserve ($\checkmark$)} & & 
\multicolumn{4}{c}{Performance} \\ \cline{3-5} \cline{7-10}
  && Hourglass & Self-attn & Cross-attn  && Chamf. & Acc. & Comp. & \textit{f}-score \\ 

\Xhline{2\arrayrulewidth}
  
1 & & $\checkmark$ &  &  &  & 1.421 & 89.897 & 81.434 & 85.105 \\ 
2 & & $\checkmark$ & $\checkmark$ &  &  &  &  & &  \\ 
3 & & $\checkmark$ &  & $\checkmark$ &  &  &  & &  \\ 
4 & & $\checkmark$ & $\checkmark$ & $\checkmark$ &  &  &  & & \\ 

\Xhline{2\arrayrulewidth}

\end{tabular}
\vspace{-2mm}
\caption{\textbf{Ablation study of architecture design in our voxel-to-point network.} Our network take two-stage approach, voxel generation network and point re-localization network. Note that Sparse hourglass indicates the voxel generation network. Self-attn and Cross-attn mean self-attention layers and cross-attention layers, respectively, in the point-localization network.}
\label{table:ablation-arch}
\end{table}

==> table/metrics/table-metric-rebuttal.tex <==
\begin{table}[!h]
\centering
\input{table/metrics/repository/after-rebuttal/full/table_shapenet}
\input{table/metrics/repository/after-rebuttal/full/table_scannet}
\input{table/metrics/repository/after-rebuttal/full/table_icl-nuim}
% \vspace{-2mm}
\caption{
\textbf{Quantitative results in ShapeNetPart, ScanNet, and ICL-NUIM datasets.} 
We measure the quality of point reconstruction from ours, point completion (PC)~\citep{pcc-snowflake}, point denoising (PD)~\citep{pcd-score} and point upsampling (PU)~\citep{pcu-dispu} using typical criteria: chamfer distance~\citep{point-recon-from-image} and percentage metric that consists of accuracy~(Acc.) and completeness~(Comp.) and $f$-score~\citep{dtu_dataset_0}.
For fair comparison, we test various conditions by changing the number of input point cloud $\mathcal{P}_\text{in}$, the upsample ratio $r$, and voxel size $l_\text{vox}$. Note that identical colors mean the results from the same pre-trained weights for each method.
}
% \label{table:metric-appendix}
% \vspace{-3mm}
\end{table}

==> table/test.tex <==
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{lcccccccccccccccccccc}

\Xhline{2\arrayrulewidth}
\multicolumn{21}{c}{ShapeNet-Part dataset} \\ 
\Xhline{2\arrayrulewidth}

\multirow{2}{*}{Methods} 
& & \multirow{2}{*}{$\mathcal{P}_\text{in}$}
& & \multirow{2}{*}{$\mathcal{P}_\text{out}$}
& & \multicolumn{3}{c}{Chamfer distance} 
& & \multicolumn{3}{c}{Percentage ($<0.5l_\text{vox}$)} 
& & \multicolumn{3}{c}{Percentage ($<l_\text{vox}$)} 
& & \multicolumn{3}{c}{Percentage ($<2l_\text{vox}$)} 

\\ \cline{7-9} \cline{11-13} \cline{15-17} \cline{19-21} 

& &  
& &  
& & k=1 & k=2 & k=4 
& & Acc. & Comp. & \textit{f}-score 
& & Acc. & Comp. & \textit{f}-score 
& & Acc. & Comp. & \textit{f}-score 
\\ 
 
\Xhline{2\arrayrulewidth}
Snowflake-PC ($r{=}4$)
& & 2048 
& & 8164
& & \first{1.12} & \first{1.32} & \second{1.61}
& & \second{80.07} & \second{30.06} & \second{41.07}
& & \second{95.93} & \first{81.76} & \second{87.53}
& & \second{99.14} & \first{98.43} & \first{98.77}
\\ 
Snowflake-PC ($r{=}4$) + Score-PD
& & 2048 
& & 8164
& & & &
& & & &
& & & &
& & & &
\\ 
Dis-PU ($r{=}4$) 
& & 2048
& & 8192
& & 1.56 & 1.69 & 1.90 
& & 60.71 & 26.91 & 36.04  
& & 86.67 & 68.19 & 75.60 
& & 96.32 & 94.19 & 95.11 
\\ 
Dis-PU ($r{=}4$) + Score-PD
& & 2048 
& & 8164
& & & &
& & & &
& & & &
& & & &
\\ 
% Ours ($l_\text{vox}{=}0.020$)
% & & 2048
% & & 8732
% & & \first{1.22} & \first{1.35} & \first{1.54}
% & & \first{81.07} & \first{40.51} & \first{53.58} 
% & & \first{96.93} & \first{81.44} & \first{88.18} 
% & & \second{99.46} & \first{93.95} & \first{96.52} 
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC__run_postech0
Ours ($l_\text{vox}{=}0.020$)
& & 2048
& & 8732
& & \second{1.19} & \second{1.33} & \first{1.52}
& & \first{81.02} & \first{40.41} & \first{53.48} 
& & \first{96.95} & \second{81.23} & \first{88.08} 
& & \second{99.46} & \first{93.90} & \second{96.49} 
% 211020__on_feat_merge__kNN_8__lr_0p001__network_transformer_self_attn_cross_attn_minkfeat__Amplitude_Cont_inv_exp_BNC_perChannel__run_postech0_23
\\ \hline

Snowflake-PC ($r{=}8$)
& & 2048 
& & 16384
& & \second{0.85} & \second{0.97} & \second{1.14}
& & 79.93 & \second{65.38} & \first{70.98}
& & \second{96.91} & \first{95.64} & \first{96.23}
& & 99.46 & \first{99.41} & \first{99.42}
\\ 
Snowflake-PC ($r{=}8$) + Score-PD
& & 2048 
& & 16384
& & 1.13 & 1.22 & 1.36
& & 65.25 & 45.44 & 52.81
& & 94.83 & 84.18 & 89.01
& & \first{99.66} & 97.45 & 98.52
\\ 
Dis-PU ($r{=}8$) 
& & 2048
& & 16384
& & {1.02} & \second{1.14} & {1.32}
& & \second{80.84} & {50.36} & {60.74}
& & {95.69} & {82.21} & 88.05
& & \second{99.57} & {96.69} & {98.07}
% 211017__up_ratio_8__network_DisPU__run_postech2_23
\\
Dis-PU ($r{=}8$) + Score-PD
& & 2048 
& & 16384
& & & &
& & & &
& & & &
& & & &
\\ 
% Dis-PU ($r{=}16$)
% & & 2048
% & & 32768
% & & {1.05} & \second{1.14}& \second{1.24}
% & & \first{90.60} & {58.51} & {65.93}
% & & 92.15 & {86.26} & {88.81}
% & & 99.26 & \first{96.88} & \first{98.01}
% % 211017__up_ratio_16__network_DisPU__run_postech1
% \\
% Ours ($l_\text{vox}{=}0.010$)
% & & 2048
% & & 15846
% & & 1.06 & 1.23 & 1.40
% & & 78.79 & \second{66.82} & \second{71.82}
% & & 94.76 & \second{87.84} & \second{90.91}
% & & 98.95 & 95.14 & 96.90
% \\
Ours ($l_\text{vox}{=}0.015$)
& & 2048
& & 15863
& & \first{0.70}  & \first{0.81}   & \first{0.92}
& & \first{85.77} & \first{69.01} & \first{78.14}
& & \first{97.11} & \second{94.98} & \second{96.16}
& & \second{99.59} & \second{99.14} & \first{99.42}
\\
\Xhline{2\arrayrulewidth}

\end{tabular}
}


